Situation Recognition with Graph Neural Networks

We address the problem of recognizing situations in images. Given an image, the task is to predict the most salient verb (action), and fill its semantic roles such as who is performing the action, what is the source and target of the action, etc. Different verbs have different roles (e.g. attacking has weapon), and each role can take on many possible values (nouns). We propose a model based on Graph Neural Networks that allows us to efficiently capture joint dependencies between roles using neural networks defined on a graph. Experiments with different graph connectivities show that our approach that propagates information between roles significantly outperforms existing work, as well as multiple baselines. We obtain roughly 3-5% improvement over previous work in predicting the full situation. We also provide a thorough qualitative analysis of our model and influence of different roles in the verbs.

==> tables/old_tables.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{ c|c c c c|c c c|c c c}
 \hline
 \multirow{2}{*}{Methods} &  \multicolumn{4}{c}{ground truth verb} & \multicolumn{3}{|c}{top-1 predicted verb} & \multicolumn{3}{|c}{top-5 predicted verbs} \\
 { } & agent & place & value & value-all & verb & value & value-all & verb & value & value-all \\
 \hline
 CNN+CRF \cite{yatskar2016imsitu} & - & - & 65.7 & 29.0 & 32.3 & 24.6 & 14.2 & 58.9 & 42.8 & 22.6 \\
 Tensor Composition \cite{yatskar2016commonly} & - & - & \textbf{70.4} & 34.4 & 34.1 & 26.5 & 15.5 & 62.6 & \textbf{46.9} & 25.5 \\
 \hline
 Chain Model & 76.0 & 69.9 & 69.7 & 45.2 & 35.4 & 26.2 & 20.3 & 61.5 & 44.6 & 32.4 \\
 Tree Model & \textbf{76.4} & \textbf{70.0} & 69.8 & \textbf{45.7} & 35.0 & 26.2 & 20.0 & 62.1 & 45.2 & 32.4 \\
 FC Graph & 76.2 & 69.7 & 69.6 & 45.4 & 34.5 & 25.8 & 19.3 & 61.6 & 45.1 & 31.7 \\
 Chain Model (BS) & 74.8 & 69.4 & 67.3 & 43.7 & 35.9 & 26.4 & 20.3 & 62.3 & 44.8 & 32.2 \\
 Tree Model (BS) & 74.9 & 69.2 & 68.1 & 44.5 & \textbf{36.2} & \textbf{26.6} & \textbf{20.6} & \textbf{62.9} & 45.1 & \textbf{32.8} \\
 \hline
\end{tabular}
\end{center}
\caption{Evaluation results on full dataset. BS inside the bracket means
beam search is used in evaluation.} \label{tab_full}
\end{table*}

\begin{table*}
\begin{center}
\begin{tabular}{ c|c c c c | c c c | c c c }
 \hline
 \multirow{2}{*}{Methods} &  \multicolumn{4}{c}{ground truth verbs} & \multicolumn{3}{|c}{top-1 predicted verb} & \multicolumn{3}{|c}{top-5 predicted verbs} \\
 { } & agent & place & value & value-all & verb & value & value-all & verb & value & value-all \\
 \hline
 Chain Model & 70.2 & 70.0 & 64.2 & 25.4 & 79.4 & 54.4 & 24.5 & \textbf{99.7} & 63.8 & 25.4 \\
 \hline
 Tree Model (1) & 76.6 & 69.7 & 67.7 & 29.1 & 80.0 & 57.3 & 28.5 & 98.9 & 67.5 & 29.1 \\
 Tree Model (2) & \textbf{78.8} & \textbf{72.6} & \textbf{69.6} & \textbf{31.7} & \textbf{80.6} & \textbf{58.6} & \textbf{30.8} & 99.1 & \textbf{69.3} & \textbf{31.6} \\
 \hline
 FC Graph (1) & 75.7 & 69.7 & 66.6 & 27.7 & 79.1 & 55.4 & 26.9 & 98.6 & 66.2 & 27.6 \\
 FC Graph (2) & 78.0 & 70.8 & 68.2 & 31.1 & 80.2 & 56.3 & 30.3 & 98.8 & 68.0 & 31.1 \\
 \hline
 FrameNet (1) & 77.1 & 70.6 & 67.7 & 28.8 & 78.8 & 56.4 & 27.9 & 98.8 & 66.9 & 28.8 \\
 FrameNet (2) & 77.1 & 71.4 & 66.7 & 26.2 & 80.0 & 54.7 & 25.6 & 98.5 & 66.2 & 26.2 \\
 \hline
\end{tabular}
\end{center}
\caption{Evaluation results on partial dataset. The numbers inside the brackets
refer to the number of updates.} \label{tab_partial}
\end{table*}



\begin{table*}
\begin{center}
\begin{tabular}{ c|c c c c | c c c | c c c }
 \hline
 \multirow{2}{*}{\#updates} &  \multicolumn{4}{c}{ground truth verbs} & \multicolumn{3}{|c}{top-1 predicted verb} & \multicolumn{3}{|c}{top-5 predicted verbs} \\
 { } & agent & place & value & value-all & verb & value & value-all & verb & value & value-all \\
 \hline
 1 & 76.3 & 69.8 & 69.5 & 45.3 & 34.5 & 25.8 & 19.7 & 60.1 & 44.0 & 31.8 \\
 2 & 76.5 & 70.7 & 69.1 & 43.8 & 34.6 & 25.6 & 18.9 & 60.7 & 44.0 & 30.9 \\
 4 & 71.3 & 66.8 & 61.2 & 31.8 & 34.6 & 22.0 & 12.5 & 60.5 & 38.1 & 21.2 \\
 6 & 64.5 & 57.1 & 50.0 & 19.4 & 34.9 & 17.1 & 6.94 & 60.7 & 30.0 & 12.0 \\
 8 & 53.1 & 43.6 & 40.2 & 11.9 & 35.4 & 13.5 & 4.03 & 61.1 & 23.7 & 6.97 \\
10 & 19.2 & 29.8 & 23.7 & 3.96 & 35.5 & 7.83 & 1.26 & 61.3 & 13.8 & 2.28 \\
 \hline
\end{tabular}
\end{center}
\caption{Evaluation results on fully-connected graph model with different number of updates.} \label{tab_diff_updates}
\end{table*}

\begin{table*}
\begin{center}
\begin{tabular}{ c|c c c c | c c c | c c c }
 \hline
 \multirow{2}{*}{Methods} &  \multicolumn{4}{c}{ground truth verbs} & \multicolumn{3}{|c}{top-1 predicted verb} & \multicolumn{3}{|c}{top-5 predicted verbs} \\
 { } & agent & place & value & value-all & verb & value & value-all & verb & value & value-all \\
 \hline
 Chain Model  & 76.0 & 69.9 & 69.7 & 45.2 & 35.4 & 26.2 & 20.3 & 61.5 & 44.6 & 32.4 \\
 Chain Model* & 74.9 & 68.4 & 64.5 & 39.2 & 36.3 & 26.5 & 19.8 & 62.4 & 43.6 & 30.6 \\
 \hline
 FC Graph  (1) & 76.3 & 69.8 & 69.5 & 45.3 & 34.5 & 25.8 & 19.7 & 60.1 & 44.0 & 31.8 \\
 FC Graph* (1) & 76.9 & 71.9 & 69.1 & 43.7 & 36.1 & 26.8 & 20.0 & 62.2 & 45.2 & 31.8 \\
 FC Graph  (2) & 76.5 & 70.7 & 69.1 & 43.8 & 34.6 & 25.6 & 18.9 & 60.7 & 44.0 & 30.9 \\
 FC Graph* (2) & 75.9 & 71.3 & 67.9 & 41.3 & 36.2 & 26.2 & 18.6 & 62.4 & 44.3 & 29.9 \\
 \hline
\end{tabular}
\end{center}
\caption{Evaluation results with different loss functions. The numbers inside the brackets refer to the number of updates and * indicates using soft logical or loss function.} \label{tab_diff_loss}
\end{table*}


